A Survey on Spatial and Spatiotemporal Prediction Methods

With the advancement of GPS and remote sensing technologies, large amounts of geospatial and spatiotemporal data are being collected from various domains, driving the need for effective and efficient prediction methods. Given spatial data samples with explanatory features and targeted responses (categorical or continuous) at a set of locations, the problem aims to learn a model that can predict the response variable based on explanatory features. The problem is important with broad applications in earth science, urban informatics, geosocial media analytics and public health, but is challenging due to the unique characteristics of spatiotemporal data, including spatial and temporal autocorrelation, spatial heterogeneity, temporal non-stationarity, limited ground truth, and multiple scales and resolutions. This paper provides a systematic review on principles and methods in spatial and spatiotemporal prediction. We provide a taxonomy of methods categorized by the key challenge they address. For each method, we introduce its underlying assumption, theoretical foundation, and discuss its advantages and disadvantages. Our goal is to help interdisciplinary domain scientists choose techniques to solve their problems, and more importantly, to help data mining researchers to understand the main principles and methods in spatial and spatiotemporal prediction and identify future research opportunities.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> biography.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in, height=1.25in, clip, keepaspectratio]{figs/zhe.jpg}}]
{Zhe Jiang} is currently an assistant professor in the department of Computer Science at the University of Alabama, Tuscaloosa. He received his Ph.D. in computer science from the University of Minnesota, Twin Cities in 2016, and B.E. in electrical engineering from the the University of Science and Technology of China, Hefei, China, in 2010. His research interests include spatial big data analytics, spatial and spatio-temporal data mining, spatial database, geographic information system, and their interdisciplinary applications in earth science, transportation, public safety, etc. He is a member of IEEE.
\end{IEEEbiography}


==> problem.tex <==
\section{Problem Statement}\label{sec:prob}
This section introduces basic concepts and formally defines the spatial classification and prediction problem. We focus on the uniqueness of spatial data and spatial classification and prediction as compared with their traditional non-spatial counterparts.

\subsection{Basic Concepts}

\emph{Spatial relationships and operations}: In GIS, the spatial relationships between two objects are categorized according to the underlying space in which the objects reside, such as set space, topological space and metric space~\cite{worboys2004gis}. Set-based spatial relationships view each spatial object as a set of points, and defines set relationships or operations such as \emph{subset of}, \emph{member of}, \emph{union} and \emph{intersection}. Topological relationships consider objects in the topological space, where each object has a boundary, interior, and exterior. One object can \emph{overlap with}, \emph{touch}, or \emph{contain} another according to whether their interior, boundary, and exterior intersect with each other. Metric space relationships consider objects in the metric space such as Euclidean space where distance and directions can be defined. The above three categories are not mutually exclusive. As shown in Figure~\ref{fig:sprelation}, the topological space is a special set space in which topological operations are  defined in addition to default set-based operations. Similarly,  the metric (e.g., Euclidean) space is a special topological space in which distance is defined in addition to default topological operations. Based on distance, more metric space operations can be defined such as direction, area, perimeter, and shape.
\begin{figure}[h]
\centering
%\includegraphics[width=1.5in]{figs/operationContain.pdf}
\subfigure[Examples of set-based, topological and metric space operations]{\includegraphics[width=1.8in]{figs/objectOperation.pdf}}
\subfigure[Relationship between objects in different spaces]{\includegraphics[width=1.5in]{figs/operationContain.pdf}}
\caption{Spatial operations on object data}
\label{fig:sprelation}
\end{figure}

For spatial field data (e.g., raster imagery), there are local, focal, zonal and global operations defined on the cells. As illustrated in Figure~\ref{fig:mapalg}, the local operators are functions on the value of a cell itself; focal operators are functions on the values of a cell together with its neighbors; zonal operators are functions on the values of a set of cells beyond a neighborhood; global operators are functions on the values of all cells. For example, computing the Normalized Digital Vegetation Index for a remote sensing imagery is a local operation because only the spectral band values of a pixel itself is used, while computing slope is a focal operation since the elevation of both current pixel and its neighbors are used. 

\begin{figure}[h]
\includegraphics[width=3in]{figs/mapalgebra.pdf}
\caption{Spatial operations on raster data (map algebra)}
\label{fig:mapalg}
\end{figure}


One important type of spatial relationship is \emph{neighborhood relationship}, which captures the range of spatial dependency between spatial data samples. Two spatial data samples are neighbors if their distance are within a threshold (for points), or their boundaries touch each other (for cells). Neighborhood relationships can be represented by an adjacency matrix called \emph{W-matrix} $W_{n\times n}$, where the element $W_{i,j}$ is non-zero when samples $i$ and $j$ are neighbors. 


\emph{Spatial learning sample}: In classification and prediction problems, data is generally viewed as a set of learning samples, and each sample is a minimum  classification or prediction unit. For spatial data, a learning sample can be a point, line, polygon, or a raster cell. Each spatial object or raster cell can be associated with a set of spatial attributes and non-spatial attributes. Spatial attributes are related to the spatial footprint of an object or a raster cell. Examples include coordinates for points or polygon centers, the length of line-strings, and the extent, area or perimeter of polygons. Non-spatial attributes are the ones that are not related to spatial footprints. Examples include the GPD of a city, the name of a river, and the age of a house. One of the non-spatial attributes is considered as the target class label or response variable, and the other non-spatial attributes together with spatial attributes are considered as explanatory features.  Thus, a spatial learning sample can generally be noted by a triplet $(x,s,y)$, where $x$ is a vector of non-spatial features, $s$ is a vector of spatial features, and $y$ is the target class label or response. 







\subsection{Problem Definition}
Given a set of spatial learning samples $(x_i,s_i,y_i)$, as well as spatial relationships between samples $R(s_i,s_j)$, $1\leq i \leq n, 1\leq j \leq n$, the spatial classification and prediction problem aims to learn a model $f$ such that $Y=f(X,R)$, where $X=(x_1, x_2,...,x_n)^T$, $Y=(y_1,y_2,...,y_n)^T$ are maps of features and target response respectively. The problem can be categorized into \emph{spatial classification} for categorical response variable and \emph{spatial prediction (or regression)} for continuous response variable. The prediction model $f$ is defined on feature maps and target response maps ($X,Y$) instead of a single sample ($x_i,y_i$) due to the existence of spatial relationships between samples. In other words, samples are not independent and identically distributed (non-i.i.d.). Moreover, the spatial relationship between samples can be of multiple kinds (both in topological space and in metric space). Such relationships are much more complicated than relationships between non-spatial data (i.e., nominal, ordinal, interval, ratio variables). Due to these reasons, classical non-spatial models are often insufficient for spatial classification and prediction problems. 



Figure~\ref{fig:appEg} shows one example of spatial classification in the application of wetland mapping. The input spatial samples are pixels in an earth observation imagery. Feature maps are spectral layers of earth imagery as shown in  Figure~\ref{fig:appEg}(a-b). The ground truth class map consists of categorical land cover types of pixels (wetland or dry land) as shown in Figure~\ref{fig:appEg}(c). Spatial relationships such as neighborhoods are established based on pixel locations. The prediction of a traditional decision tree classifier are shown in Figure~\ref{fig:appEg}(d). Compared with the ground truth class map, decision tree predictions have lots of artifacts (e.g., salt-and-pepper noise), requiring tedious and time-consuming post-processing. The reason is that decision trees ignore the spatial relationships between samples, and classify each sample independently from each other. This is a general issue for other model families such as maximum likelihood classifiers, neural networks, and support vector machines. Thus, spatial classification methods are needed.


It is worth noting that in our definition of spatial prediction, the response variable $y$ is a non-spatial attribute at fixed locations. This does not include problems in which the response variable $y$ is a spatial location (i.e., locations are random variables). Examples of such problems are location prediction and location recommendation for moving object data, which have been extensively studied in the data mining literature. Due to space limit, these problems are not included in the survey.
